Deep Tensor Factorization for Spatially-Aware Scene Decomposition

We propose a completely unsupervised method to understand audio scenes observed with random microphone arrangements by decomposing the scene into its constituent sources and their relative presence in each microphone. To this end, we formulate a neural network architecture that can be interpreted as a nonnegative tensor factorization of a multi-channel audio recording. By clustering on the learned network parameters corresponding to channel content, we can learn sources' individual spectral dictionaries and their activation patterns over time. Our method allows us to leverage deep learning advances like end-to-end training, while also allowing stochastic minibatch training so that we can feasibly decompose realistic audio scenes that are intractable to decompose using standard methods. This neural network architecture is easily extensible to other kinds of tensor factorizations.

==> changes.tex <==
% Cross things out if you’ve fixed them.
% Original as a zip
% Overleaf
% We can edit into the overleaf. I made a copy^^ and made a duplicate folder in the overleaf itself.
% ======= Review 1 =======
% > *** Recommended Changes: Comments to the author: Please indicate any changes that should be made to the paper if it is accepted.

% Fill in additional details on network setup and acoustic simulation parameters. Check and fix details in bibliography. Add units to figures.

% -IDK what additional details they want….
% -IDK what details in the bib they want….
% -The only units we’re missing is dB on the SDR SIR SAR, I’ll add those if we keep the figures the same.

% > *** Weaknesses: Comments to the author: what are the weak aspects of the paper?

% Results show a significant variation across simulation runs, which is expected, that depending on setup results may results in degradation. Visualization or audio samples of extracted sources are unfortunately missing.

% -I don’t think they noticed the link to our demo website which has sample factorizations for each kind of scene.

% ======= Review 2 =======
% > *** Recommended Changes: Comments to the author: Please indicate any changes that should be made to the paper if it is accepted.

% - Figures 3, 4, and 5 are useful, but it is difficult to compare the absolute numbers on the vertical scale. A small table with numbers will help and will not take much space. 
% - References [3] [11], [13], and [16] are missing capitalization in the paper titles (hint: use {}).

% I can make the table with numbers
% Fixed capitalization in titles for the bibliography

% > *** Weaknesses: Comments to the author: what are the weak aspects of the paper?

% The paper is missing baseline. There is no comparison with already published similar algorithm, the results from the proposed two versions of the algorithm are presented "as is". The improvement is not clear even in absolute numbers because of the vertical scale of figures 3, 4, and 5.

% -Not about to do a baseline and so all we’re gonna change is the table units. 

% ======= Review 3 =======
% - Some thoughts on expected real-world behaviour would be beneficial.
% - Comment on the array configurations question below.
% - Sec.2.3.1: "We recover a single channel recording ...Wiener filters.", that's a bit vague, please be more specific.
% - Sec.3: "As for ambient source...", explain how ambient sources were rendered? Was the same signal replicated to the virtual microphones (coherently?) Was there any decorrelation applied between channels as realistic ambient sources would be?
% - Sec.3: "This tests wether the model can ...", give some more information how this ambiguity is controlled - where the ambient sources coherent? equal power across channels?
% - Sec.4: "of decomposing reverberant audio scenes", up-to-two order image sources is not reverberation, for such a claim to be made.

% -Not sure what commentary they want here?
% -This really is application heavy. It is true though that we rely on spatial uniqueness. We can make a comment about being able to run our model after a beamformer.
% - Ah yeah, we can do this.
% -Mention they are added
% -This is a good point, we should also mentioned the played with 0 SNR thing.
% -Ouch. I really have no idea if this is true or not.

% > *** Weaknesses: Comments to the author: what are the weak aspects of the paper?

% The main weakness of the paper is no evaluation with any real data at all, however, the three fundamental scene configurations that were evaluated were convincing and clear for a first theoretical evaluation.

% Another thing that is not mentioned at all is the non-negative part of the factorization - in essence it is suitable for only non-negative real weights across the channels which would be suitable for the widely distributed spatially diverse arrays that are used in the study, where the source images can have significant energy differences across channels due to propagation attenuation. That would exclude a class of common arrays such as small spaced arrays with the sources being around and in the far field of the array, where complex weights (phase differences) capture most of the spatial diversity. What happens even in the widely spaced case if the microphones are directional, as is quite common in real life? Additionally, there are coincident spatial sound recording setups with both positive and negative directional responses (e.g. figure-of-eight microphones or ambisonic recording)/ Please comment on these considerations in the text.

